Database-assisted Distributed Spectrum Sharing

According to FCC's ruling for white-space spectrum access, white-space devices are required to query a database to determine the spectrum availability. In this paper, we study the database-assisted distributed white-space access point (AP) network design. We first model the cooperative and non-cooperative channel selection problems among the APs as the system-wide throughput optimization and non-cooperative AP channel selection games, respectively, and design distributed AP channel selection algorithms that achieve system optimal point and Nash equilibrium, respectively. We then propose a state-based game formulation for the distributed AP association problem of the secondary users by taking the cost of mobility into account. We show that the state-based distributed AP association game has the finite improvement property, and design a distributed AP association algorithm that can converge to a state-based Nash equilibrium. Numerical results show that the algorithm is robust to the perturbation by secondary users' dynamical leaving and entering the system.

==> UserAlg.tex <==
\section{\label{sec:Distributed-AP-Association}Distributed AP Association
Algorithm}

We next design a distributed AP association algorithm based on the
finite improvement property shown in Theorem \ref{thm:The-distributed-AP},
which allows secondary users to select their associated APs in a distributed
manner and achieve mutually acceptable AP associations, i.e., a state-based Nash
equilibrium.

The key idea is to let secondary users asynchronously improve their
AP selections. Unlike the deterministic AP channel selection update
with the fixed order enforced by the geo-location database, the distributed AP
association algorithm can not be deterministic. This is because that, as secondary users dynamically enter and leave the network, a deterministic distributed AP association
algorithm according to the fixed strategy update order is not robust.
Hence we will design a randomized algorithm by letting each
secondary user countdown according to a timer value that follows the
exponential distribution with a mean equal to $\eta$. Since the exponential distribution has support over $(0,\infty)$ and its probability density function is continuous,
the probability that more than one users generate the same timer value
and update their strategies simultaneously equals zero.\footnote{The timer in practice is always finite, and the collision probability is not exactly zero. However, as long as the collision probability is very small, the following analysis is a very good approximation of the reality.} When a user
$k$ activates its strategy update at time $t$, the user can computes
its best response strategy as \begin{eqnarray}
b_{k}^{*} & = & \arg\max_{b_{k}}V_{k}(b_{k},b_{-k}^{t},\boldsymbol{s}^{t})\nonumber \\
 & = & \arg\max_{b_{k}}H_{k}U_{b_{k}}(\boldsymbol{a}^{*})g(x_{b_{k}}(\boldsymbol{b}^{t}))-\delta_{k}d_{b_{k}s_{k}},\label{eq:ss0}\end{eqnarray}
which requires the information of user distribution $(x_{1}(\boldsymbol{b}^{t}),...x_{N}(\boldsymbol{b}^{t}))$
at time $t$, the throughput $U_{n}(\boldsymbol{a}^{*})$ and geo-locations of
all the APs.

To facilitate the best response update, we propose to
setup a social database (accessible by all secondary users), wherein
each AP reports its channel throughput $U_{n}(\boldsymbol{a}^{*})$ and geo-location,
and each secondary user $k^{'}\in\mathcal{K}$ posts and shares its
AP association $b_{k^{'}}^{*}$ with other users in the manner like
Twitter once it updates. Based on the information from the social
database, a secondary user $k$ can first figure out the user distribution
$(x_{1}(\boldsymbol{b}^{t}),...x_{N}(\boldsymbol{b}^{t}))$ as \begin{equation}
x_{n}(\boldsymbol{b}^{t})=\sum_{k^{'}=1}^{K}I_{\{b_{k'}^{t}=n\}},\forall n\in\mathcal{N},\label{eq:ss1}\end{equation}
where $I_{\{b_{k'}^{t}=n\}}=1$ if user $k'$ associates with AP $n$,
and $I_{\{b_{k'}^{t}=n\}}=0$ otherwise. Based on the user distribution,
the secondary user $k$ can then compute the corresponding best response
strategy according to (\ref{eq:ss0}).

The success of social database requires that each user is willing
to share the information of its AP association. When this
is not feasible, each AP $n$ can estimate its associated user population $x_{n}$
locally. Let $\bar{g}(x_{n})$ denote the probability that no user
among $x_{n}$  associated with the same AP grabs the channel in a time slot
$\tau$. This can be computed as $\bar{g}(x_{n})=1-x_{n}g(x_{n})$,
where $g(x_{n})$ is given in (\ref{eq:gg}). In a time slot $\tau$, AP $n$
can observe the information $I_{a_{n}^{*}}(\tau)\in\{1,0\}$, i.e., whether the channel $a_{n}^{*}$ is used by any users or not. Then
over a long period that consists of $L$ time slots, AP $n$ can observe
the outcome $\{I_{a_{n}^{*}}(\tau)\}_{\tau=1}^{L}$ and estimate $\bar{g}(x_{n})=\frac{\sum_{\tau=1}^{L}I_{a_{n}^{*}}(\tau)}{L}$
by the sample-average. Since $I_{a_{n}^{*}}(\tau)$ is independently
and identically distributed according to the probability $\bar{g}(x_{n})$,
according to the law of large number, the estimation will be accurate when the observation period length $L$ is large enough.
This is feasible in practices since user's mobility decision is often
carried out at a large time scale (say every few minutes), compared
with the time scale of a time slot (say $50$ microseconds in the
standard 802.11 system). Then AP $n$ can obtain the number of its
associated users $x_{n}$ by solving that $x_{n}=\bar{g}^{-1}\left(\frac{\sum_{\tau=1}^{L}I_{a_{n}^{*}}(\tau)}{L}\right)$, and report it in the social database.

We summarize the distributed
AP association algorithm in Algorithm \ref{alg:-Distributed-AP}.
According to Theorem \ref{thm:For-the-distributed}, such asynchronous
best response update process must reach a state-based Nash equilibrium.
Numerical results show that the algorithm is also robust to the dynamics
of secondary users' leaving and entering the system.


\begin{algorithm}[tt]
\begin{algorithmic}[1]
\State \textbf{initialization:}
\State \hspace{0.4cm} \textbf{set} the mean $\eta$ for strategy update countdown.
\State \textbf{end initialization\newline}

\Loop{ for each secondary user $k\in\mathcal{K}$ in parallel:}
        \State \textbf{generate}  a timer value that follows the exponential distribution
with the mean $\eta$.
        \State \textbf{count down} until the timer expires.
        \If{ the timer expires}
            \State \textbf{acquire} the information of channel throughput $\{U_{n}(\boldsymbol{a}^{*})\}$, the geo-location of APs, and user distribution $\{x_{n}\}_{n=1}^{N}$.
            \State \textbf{update} the strategy $b_{k}^{*}$ according to the best response in (\ref{eq:ss0}).
        \EndIf
\EndLoop
\end{algorithmic}
\caption{\label{alg:-Distributed-AP} Distributed AP Association Algorithm}
\end{algorithm} 
